Robust Calibration with Multi-domain Temperature Scaling

Uncertainty quantification is essential for the reliable deployment of machine learning models to high-stakes application domains. Uncertainty quantification is all the more challenging when training distribution and test distribution are different, even the distribution shifts are mild. Despite the ubiquity of distribution shifts in real-world applications, existing uncertainty quantification approaches mainly study the in-distribution setting where the train and test distributions are the same. In this paper, we develop a systematic calibration model to handle distribution shifts by leveraging data from multiple domains. Our proposed method -- multi-domain temperature scaling -- uses the heterogeneity in the domains to improve calibration robustness under distribution shift. Through experiments on three benchmark data sets, we find our proposed method outperforms existing methods as measured on both in-distribution and out-of-distribution test sets.

==> problemsetup.tex <==
\newpage
\section{Problem setup}\label{sec:problemsetup}
We denote the input space and the label set by $\mathcal{X}$ and $\mathcal{Y}$. We consider the multiple task scenario, and let $\mathscr{D}_{k}$ denote the distribution for $k$-th task on input space $\mathcal{X}$ for $k\in[K]$.  Let $f: \mathcal{X} \rightarrow \mathcal{Y}$  denote the classifier where $\hat{Y}=f(X)$, $\hat{Y}\in\mathcal{Y}$, and $X\in \mathcal{X}$. We assume there exists a classifier $f^{\star}$ that correctly predicts inputs from $\mathcal{X}$ regardless of tasks, i.e., $Y=f^{\star}(X)$ for $X\in\mathcal{X}$. For the $k$-th task,  we use $h^{\star}_{k}(\cdot; f): \mathcal{X}\rightarrow[0, 1]$ to denote the true calibration map associated with classifier $f$, i.e., $\mathbb{P}[\hat{Y}=Y|\hat{P}=p]=p,\,\,\forall p\in[0, 1]$,  where $\hat{Y}=f(X)$,  $\hat{P}=h^{\star}_{k}(X; f)$, and $X \sim \mathscr{D}_{k}$. 


We focus on the setting when the classifier $\hat{f}$ is learned and fixed, we aim to learn $\hat{h}\in\mathscr{H}$ such that $\varepsilon(\hat{h}, \mathscr{D}_{k}) = \mathbb{E}_{X\sim\mathscr{D}_{k}}[|{h}^{\star}_{k}(X)-\hat{h}(X)|]$ is small for every task $k$, where $\varepsilon_k(\hat{h})$ is the error of $\hat{h}$ on $\mathscr{D}_{k}$. Meanwhile, we are interested in generalizing to new tasks: suppose there is an unseen out-of-distribution task $\widetilde{\mathscr{D}}$ which can be different from existing tasks, i.e., $\widetilde{\mathscr{D}}(X) \neq {\mathscr{D}_k}(X)$ for $k\in[K]$. 
Our goal is to learn $\hat{h}$ that achieves similar calibration performance on the  out-of-distribution task as in-distribution tasks, $\varepsilon(\hat{h}, \widetilde{\mathscr{D}})\leq \varepsilon(\hat{h}, \mathscr{D}_{k}) + \gamma$ and $\gamma\geq 0$, when the distance between $\widetilde{\mathscr{D}}$ and the mixture of $\{\mathscr{D}_k\}_{k=1}^{K}$ is not large. To define the distance between two distributions, we first introduce the  $\mathscr{H}$-divergence~\citep{ben2010theory} to measure the distance between two distributions:

% \vspace{-0.05in}
\begin{definition}[$\mathscr{H}$-divergence]
Given an input space $\mathcal{X}$ and two probability distributions $\mathscr{D}$ and $\mathscr{D}^{\prime}$ on $\mathcal{X}$, let $\mathscr{H}$ be a hypothesis class on  $\mathcal{X}$, and denote by $\mathscr{A}$ the collection of subsets of $\mathcal{X}$ which are the support of hypothesis $h\in\mathscr{H}$, i.e., $\mathscr{A}_{\mathscr{H}}=\{h^{-1}(1)\,|\,h\in\mathscr{H}\}$. The distance between $\mathscr{D}$ and $\mathscr{D}^{\prime}$ is 
\begin{equation}\label{eq:def-H-divergence}
    \mathrm{d}_{\mathscr{H}}(\mathscr{D}, \mathscr{D}^{\prime}) = \sup_{A\in\mathscr{A}_{\mathscr{H}}} \left|\mathrm{Pr}_{\mathscr{D}}(A)-\mathrm{Pr}_{\mathscr{D}^{\prime}}(A)\right|.
\end{equation}
\end{definition}
\vspace{-0.1in}
The $\mathscr{H}$-divergence reduces to the standard total variation (TV) distance when $\mathscr{H}$ contains all measurable functions on $\mathcal{X}$, which implies that the $\mathscr{H}$-divergence is upper bounded by the TV-distance, i.e., $\mathrm{d}_{\mathscr{H}}(\mathscr{D}, \mathscr{D}^{\prime}) \leq \mathrm{d}_{{\scriptsize \textsf{TV}}}(\mathscr{D}, \mathscr{D}^{\prime})$. 
On the other hand, when the hypothesis class $\mathscr{H}$ has a finite VC-dimension or pseudo-dimension, the $\mathscr{H}$-divergence can be estimated using finite samples from $\mathscr{D}$ and $\mathscr{D}^{\prime}$~\citep{ben2010theory}. Next, we define the mixture distribution of the $K$ in-distribution tasks $\mathscr{D}_{K}^{\alpha}$ on input space $\mathcal{X}$ as 
\vspace{-0.05in}
\begin{equation}\label{eq:def-mixture-dist}
    \mathscr{D}_{K}^{\alpha} = \sum_{k=1}^{K} \alpha_{k} \mathscr{D}_{k}, \quad \sum_{k=1}^{K}\alpha_{k} = 1\,\,\textrm{and}\,\,\alpha_{k}\geq 0.
\end{equation}
Previous work~\citep{zhao2018adversarial} developed the generalization bound on the out-of-distribution risk that depends on the in-distribution risk as well as the discrepancy between in-distribution $\mathscr{D}$ and out-of-distribution distribution $\widetilde{\mathscr{D}}$:

\vspace{-0.05in}
\begin{theorem}[\citet{zhao2018adversarial}]\label{theorem:regression-bound-population}
Let $\mathscr{H}$ be the hypothesis class contains functions $h:\mathcal{X}\rightarrow [0, 1]$, and denote the in-distribution by $\mathscr{D}$ and out-of-distribution $\widetilde{\mathscr{D}}$. Then for any $h\in\mathscr{H}$, we have
\begin{equation}\label{eq:theorem-regression}
    \varepsilon(h, \widetilde{\mathscr{D}}) \leq \varepsilon(h, {\mathscr{D}}) + \frac{1}{2}\mathrm{d}_{\bar{\mathscr{H}}}(\mathscr{D}, \widetilde{\mathscr{D}}) + \underbrace{\varepsilon(h^{\star}, \mathscr{D}) + \varepsilon(h^{\star}, \widetilde{\mathscr{D}})}_{\lambda(\mathscr{D}, \widetilde{\mathscr{D}})},
\end{equation}

\vspace{-0.15in}
where $h^{\star} := \mathrm{argmin}_{h\in\mathscr{H}} \{\varepsilon(h, \mathscr{D}) + \varepsilon(h, \widetilde{\mathscr{D}})\}$ and $\bar{\mathscr{H}}$ is defined as $\bar{\mathscr{H}}:= \{\mathrm{sign}(|h(x) - h^{\prime}(x)| - t)\,|\,h, h^{\prime}\in\mathscr{H}, 0 \leq t \leq 1\}$.
\end{theorem}
We provide the proof of Theorem~\ref{theorem:regression-bound-population} in Appendix~\ref{sec:appendix-miss-proof} for completeness. We can decompose the upper bound into two parts: (1). Risk of $h$ on the in-distribution $\mathscr{D}$, $\varepsilon(h, {\mathscr{D}})$; (2). Discrepancy between two distributions and the combined risk of the optimal hypothesis on $\mathscr{D}$ and $\widetilde{\mathscr{D}}$, $\frac{1}{2}\mathrm{d}_{\bar{\mathscr{H}}}(\mathscr{D}, \widetilde{\mathscr{D}}) + \lambda(\mathscr{D}, \widetilde{\mathscr{D}})$. The second part does not depend on the choice of hypothesis $h$, which only depends on $\mathscr{D}$ and $\widetilde{\mathscr{D}}$. On the other hand, given multiple tasks $\{\mathscr{D}_1, \dots, \mathscr{D}_{K}\}$, we can optimize the combination parameters $\alpha$ such that $\mathscr{D}_{K}^{\alpha}$ minimizes the second part. More specifically, we have
\begin{equation}\label{eq:optimize-alpha}
    \hat{\alpha} = \underset{\alpha \in \Delta^{K-1}}{\mathrm{argmin}} \left\{\frac{1}{2}\mathrm{d}_{\bar{\mathscr{H}}}(\mathscr{D}_{K}^{\alpha}, \widetilde{\mathscr{D}}) + \lambda(\mathscr{D}_{K}^{\alpha}, \widetilde{\mathscr{D}})\right\}.
\end{equation}
Therefore, from Eq.~\eqref{eq:theorem-regression} and Eq.~\eqref{eq:optimize-alpha}, we find that using multiple tasks ($\mathscr{D}^{\hat{\alpha}}_K$) can lead to improved performance compared with the single task $(\mathscr{D})$  if $|\inf_{h\in\mathscr{H}}\varepsilon(h, {\mathscr{D}})-\inf_{h^{\prime}\in\mathscr{H}}\varepsilon(h^{\prime}, {\mathscr{D}^{\hat{\alpha}}_K})|$ is relatively small. Meanwhile, the risk of the hypothesis $h$ on the mixture distribution $\mathscr{D}^{\hat{\alpha}}_K$ can be represented as the convex combination of the risk on every task, i.e., $\varepsilon(h, {\mathscr{D}^{\hat{\alpha}}_K}) = \sum_{k=1}^{K}\hat{\alpha}_k\cdot\varepsilon(h, {\mathscr{D}_k})$. We now give a upper bound on the risk on OOD. The proof are mainly based on results from \citet{blitzer2007learning, zhao2018adversarial} and the proof details can be found in Appendix~\ref{sec:appendix-miss-proof}.

\vspace{-0.05in}
\begin{theorem}\label{theorem:regression-bound-OOD}
Let $\mathscr{H}$ be the hypothesis class contains functions $h:\mathcal{X}\rightarrow [0, 1]$ with psuedo-dimension $\mathrm{Pdim}(\mathscr{H})=d$. $\{S_{k}\}_{k=1}^{K}$ are the empirical distributions generated from $\{\mathscr{D}_k\}_{k=1}^{K}$, where $S_{k}$ contains $n$ i.i.d. samples from $\mathscr{D}_k$. If $\varepsilon(\hat{h}, {\mathscr{D}_k}) \leq \varepsilon({h}_k^{\star}, {\mathscr{D}_k}) + \gamma$, then for $\delta \in (0, 1)$, with probability at least $1-\delta$, we have
\vspace{-0.1in}
\begin{equation}\label{eq:theorem-regression-ood}
    \varepsilon(\hat{h}, \widetilde{\mathscr{D}}) \leq \gamma +  \sum_{k=1}^{K}\hat{\alpha}_{k}\cdot\hat{\varepsilon}({h}_k^{\star}, {\mathscr{D}_k}) + \frac{1}{2}\mathrm{d}_{\bar{\mathscr{H}}}(\mathscr{D}^{\hat{\alpha}}_K, \widetilde{\mathscr{D}}) + \lambda(\mathscr{D}^{\hat{\alpha}}_K, \widetilde{\mathscr{D}}) + \widetilde{O}\left(\frac{\mathrm{Pdim}(\mathscr{H})}{\sqrt{nK}}\right),
\end{equation}

\vspace{-0.15in}
where $\hat{\alpha}$ is defined in Eq.~\eqref{eq:optimize-alpha}, $\mathrm{Pdim}(\mathscr{H})$ is the psuedo-dimension of the hypothesis class $\mathscr{H}$, and $\hat{\varepsilon}({h}, S_k)$ is the empirical risk of the hypothesis $h$ on $S_k$.
\end{theorem}
\vspace{-0.15in}
\begin{remark}
Suppose we can learn hypothesis $\hat{h}$ achieves similar risk as the optimal hypothesis ${h}^{\star}_{k}$ on every task, then $\hat{h}$ is able to achieve improved performance on the OOD data through leveraging the multiple task structure. In other words, if the learned calibration map $\hat{h}$ is well-calibrated on every task, then $\hat{h}$ is likely to provide calibrated confidences when the new task is similar to the mixture distribution of existing tasks measure by $\mathscr{H}$-divergence.
\end{remark}


\vspace{-0.05in}
Motivated by results in Theorem~\ref{theorem:regression-bound-OOD}, we develop a practical method in Section~\ref{sec:method} to learn the calibration map $\hat{h}$ such that $\hat{h}$ is well-calibrated on every available task. 

